Restricting Representations from a Complex Group to a Real Form

Let $G$ be a complex connected reductive algebraic group and let $G_{\mathbb{R}}$ be a real form of $G$. We construct a sequence of functors $L_i\mathcal{R}$ from admissible (resp. finite-length) representations of $G$ to admissible (resp. finite-length) representations of $G_{\mathbb{R}}$. We establish many basic properties of these functors, including their behavior with respect to infinitesimal character, associated variety, and restriction to a maximal compact subgroup. We deduce that each $L_i\mathcal{R}$ takes unipotent representations of $G$ to unipotent representations of $G_{\mathbb{R}}$. Taking the alternating sum of $L_i\mathcal{R}$, we get a well-defined homomorphism on the level of characters. We compute this homomorphism in the case when $G_{\mathbb{R}}$ is split.

==> scratch.tex <==


\section{The associated graded of a principal series representation}

Assume in this section that $G_{\RR}$ is quasi-split. Fix a maximally split Cartan subgroup $H_{\RR} \subset G_{\RR}$ with Cartan decomposition
%
$$H_{\RR} = T_{\RR}A_{\RR}$$
%
Fix a real Borel subgroup $B_{\RR} = H_{\RR}N_{\RR}$ of $G_{\RR}$. Characters of $H_{\RR}$ are in bijection with pairs
%
$$(\overline{\delta}, \nu) \in \widehat{T}_{\RR} \times \widehat{A}_{\RR} \simeq X^*(H)/(1-\sigma_c) \times \mathfrak{a}^*$$
%
Write $\CC(\overline{\delta},\nu)$ for the character of $H_{\RR}$ corresponding to the pair $(\overline{\delta},\nu)$. Note that the infinitesimal character of $\CC(\overline{\delta},\nu)$ is 
%
$$\lambda=\frac{1}{2}(1+\sigma_c)\delta + \nu \in \fh^*$$
%
Consider the principal series representation of $G_{\RR}$
%
$$I_{\RR}(\overline{\delta},\nu) := \Ind^{G_{\RR}}_{B_{\RR}} \CC(\overline{\delta},\nu), \qquad \text{(normalized parabolic induction)}.$$
%
Our goal in this section is to compute the class $\gr [I_{\RR}(\overline{\delta},\nu)] \in K^K(\cN_{\theta})$. 

Let $X$ be the flag variety for $G$, $\pi: T^*(X) \to X$ the projection and $p: T^*(X) \to \fg^*$ the Springer map. Since $p$ is proper, there is a group homomorphism
%
$$p_*: K^G(T^*(X)) \to K^G(\fg^*), \qquad p_*[\mathcal{E}] = \sum_i (-1)^i [R^ip_*(\mathcal{E})]$$
%
Let $U \subset X$ be the $K$-orbit of $B$ and let $j: U \hookrightarrow X$ be the inclusion. Note that $U$ is the (unique) open $K$-orbit on $X$. Form the sheaf $\mathcal{D}_X^{\lambda-\rho}$ of twisted differential operators on $X$, and let $\mathcal{D}_U^{\lambda-\rho}$ be the restriction of $\mathcal{D}_X^{\lambda-\rho}$ to $U$. Then the category $M(\mathcal{D}_U^{\lambda-\rho},K)$ of $K$-equivariant $\mathcal{D}_U^{\lambda-\rho}$-modules on $U$ is equivalent to the category of $(\fh,T)$-modules on which $\fh$ acts by $\lambda-\rho$. Let $\tau_U(\overline{\delta},\nu)$ be the irreducible $K$-equivariant  $\mathcal{D}_U^{\lambda-\rho}$-module corresponding to the $(\fh,T)$-module $\CC(\overline{\delta},\nu) \otimes |\rho(\fn)|^{-1}$. Then

\begin{prop}\label{prop:BB}
Suppose $\lambda$ is weakly dominant for $\Delta(\fh,\fb)$. Then:
\begin{itemize}
    \item[(i)] The functor $\Gamma: M(\mathcal{D}_X^{\lambda-\rho},K) \to M(\fg,K)$ is exact.
    \item[(ii)] $\Gamma(X,j_!\tau_U(\overline{\delta},\nu)) \simeq I_{\RR}(\overline{\delta},\nu)$.
\end{itemize}
\end{prop}

There is a group homomorphism
%
$$\gr: KM(\mathcal{D}_X^{\lambda-\rho},K) \to K^K(T^*(X))$$

\begin{lemma}\label{lem:1}
There is an identity in $K^K(\cN_{\theta})$
%
$$\gr[I_{\RR}(\overline{\delta},\nu)] = p_* \gr[j_!\tau_U(\overline{\delta},\nu)]$$
\end{lemma}

\begin{proof}
First note that $[I_{\RR}(\overline{\delta},\nu)] \in KM(\fg,K)$ is independent of the choice of Borel subgroup $B_{\RR}$. So we can assume without loss that $\lambda$ is weakly dominant for $\Delta(\fh,\fb)$. 

Now by Proposition \ref{prop:BB}, there is an identity in $KM(\fg,K)$
%
$$[I_{\RR}(\overline{\delta},\nu)] = \sum_i (-1)^i [H^i(X,j_!\tau_U(\overline{\delta},\nu))]$$
%
and hence an identity in $K^K(\cN_{\theta})$
%
$$\gr[I_{\RR}(\overline{\delta},\nu)] = \sum_i (-1)^i \gr[H^i(X,j_!\tau_U(\overline{\delta},\nu))]$$
%
By a standard spectral sequence argument (see Lemma \ref{lem:spectral})
%
\begin{align*}\sum_i (-1)^i \gr[H^i(X,j_!\tau_U(\overline{\delta},\nu))] &= \sum_i (-1)^iR^ip_* \gr[j_!\tau_U(\overline{\delta},\nu)]\\
&= p_*\gr[j_!\tau_U(\overline{\delta},\nu)]\end{align*}
%
The lemma follows.
\end{proof}

\begin{lemma}\label{lem:2}
There is an identity in $K^K(T^*(X))$
%
$$\gr[j_!\tau_U(\overline{\delta},\nu)] = [\pi^*\OO_X(\delta)] \otimes \gr[j_!\tau_U(0,\nu)].$$
\end{lemma}

\begin{proof}
Since the functor $j_!$ is local with respect to the target variety, it commutes with line bundle twists, i.e. there is an isomorphism in $M(\mathcal{D}^{\lambda-\rho},K)$
%
$$j_!\tau_U(\overline{\delta},\nu) \simeq  \cO_X(\delta) \otimes j_!\tau_U(0,\nu)$$
%
Thus
%
$$\gr[j_!\tau_U(\overline{\delta},\nu)] = \gr[\cO_X(\delta) \otimes j_!\tau_U(0,\nu)]$$
%
Let $F_mj_!\tau_U(0,\nu)$ be a good filtration of $j_!\tau_U(0,\nu)$. Then $\cO_X(\delta) \otimes F_mj_!\tau_U(0,\nu)$ is a good filtration of $\cO_X(\delta) \otimes j_!\tau_U(0,\nu)$. For each $m$, we have
%
$$(\cO_X(\delta) \otimes F_mj_!\tau_U(0,\nu))/(\cO_X(\delta) \otimes F_{m-1}j_!\tau_U(0,\nu))\simeq \pi^*\cO_X(\delta) \otimes \gr_m j_!\tau_U(0,\nu)$$
%
So
%
$$\gr[j_!\tau_U(\overline{\delta},\nu)] = [\pi^*\cO_X(\delta)] \otimes \gr[j_!\tau_U(0,\nu)]$$
%
as required.
\end{proof}

\begin{theorem}[Dougal-Vilonen]\label{thm:DougalVilonen}
There is an identity in $K^K(T^*(X))$
%
$$\gr[j_!\tau_U(0,0)] = [p^*\cO_{\fp^*}].$$
\end{theorem}

\begin{theorem}\label{thm:grprincipal}
There is an identity in $K^K(\cN_{\theta})$
%
$$\gr[I_{\RR}(\overline{\delta},\nu)] = p_*([\pi^*\cO_X(\delta)] \otimes [p^*\cO_{\fp^*}])$$
\end{theorem}

\begin{proof}
The class $\gr[I_{\RR}(\overline{\delta},\nu)]$ is independent of $\nu$, see \cite[(3), p. 54]{AdamsVoganAV}. In particular
%
\begin{equation}\label{eq:prinseries1}\gr[I_{\RR}(\delta,\nu)] = \gr[I_{\RR}(\delta,0)]\end{equation}
%
Combining Lemmas \ref{lem:1} and \ref{lem:2}, we obtain
%
\begin{equation}\label{eq:prinseries2}\gr[I_{\RR}(\delta,0)] = p_*([\pi^*\cO_X(\delta)] \otimes \gr[j_!\tau_U(0,0)])\end{equation}
%
Substituting the statement of Theorem \ref{thm:DougalVilonen} into Equation (\ref{eq:prinseries2}), we obtain
%
\begin{equation}\label{eq:prinseries3}\gr[I_{\RR}(\delta,0)] = p_*([\pi^*\cO_X(\delta)] \otimes [p^*\cO_{\fp^*}])\end{equation}
%
The result now follows immediately from (\ref{eq:prinseries1}) and (\ref{eq:prinseries3}).
\end{proof}

\section{Case of split groups}\label{sec:principal series}

Now assume that $G_{\RR}$ is \emph{split}. Fix a split maximal torus $H \subset G$ and a Borel subgroup $B=HN \subset G$. Write $H_{\RR} \subset G_{\RR}$ and $B_{\RR} \subset G_{\RR}$ for the groups of real points. Let 
%
$$H= TA$$
%
be the Cartan decomposition of $H$. Here, $T$ is a product of circle groups and $A$ is a complex vector group. Let $T_{\RR} = T \cap H_{\RR}$ and $A_{\RR} = A \cap H_{\RR}$. Then $T_{\RR}$ is a product of cyclic groups of order 2, $A_{\RR}$ is a real vector group, and
%
$$H_{\RR} = T_{\RR}A_{\RR}$$
%
is the Cartan decomposition of $H_{\RR}$. Characters of $H$ are in bijection with pairs of the form
%
$$(\lambda, \nu) \in \widehat{T} \times \widehat{A} \simeq  X^*(H) \times \fh^*,$$
%
and characters of $H_{\RR}$ are in bijection with pairs of the form
%
$$(\overline{\lambda}, \nu) \in \widehat{T}_{\RR} \times \widehat{A}_{\RR} \simeq X^*(H)/(1-\sigma_c) \times \fh^*$$
%
Write $\CC(\lambda,\nu)$, resp. $\CC(\overline{\lambda},\nu)$, for the corresponding characters. Denote the principal series of $G$ and $G_{\RR}$ by
%
$$I_{\CC}(\lambda, \nu) := \Ind^G_B \CC(\lambda,\nu), \qquad I_{\RR}(\overline{\lambda},\nu) := \Ind^{G_{\RR}}_{B_{\RR}} \CC(\overline{\lambda},\nu).$$
%
Recall that $KM_{fl}(G)$ is spanned by the classes $[I_{\CC}(\lambda,\nu)]$. So to compute the homomorphism $\mathcal{R}: KM_{fl}(G) \to KM_{fl}(G_{\RR})$ it suffices to compute the classes $\mathcal{R} [I_{\CC}(\lambda,\nu)]$ for each $(\lambda,\nu)$. In fact, we will prove the following.

\begin{theorem}\label{thm:principalseries}
For each $(\lambda, \nu) \in X^*(H) \times \fh^*$ there is an identity in $KM_{fl}(G_{\RR})$
%
$$\mathcal{R} [I_{\CC}(\lambda,\nu)] = [I_{\RR}(\overline{\lambda},\nu)].$$
\end{theorem}

First, we will show that Theorem \ref{thm:principalseries} holds on the level of coherent sheaves. 


There is a Cartesian diagram
%
\begin{center}
    \begin{tikzcd}
    T_{\theta}^*(X \times X) \ar[r,"p"] & \cN\\
    T_{\theta}^*(X) \ar[r,"p"] \ar[u,hookrightarrow,"\iota"]& \cN_{\theta} \ar[u,hookrightarrow,"i"]
    \end{tikzcd}
\end{center}


\begin{lemma}
The following diagram commutes
%
\begin{center}
    \begin{tikzcd}
K^G(T_{\theta}^*(X \times X)) \ar[r,"p_*"] \ar[d,"\iota^*"] & K^G(\cN) \ar[d,"i^*"] \\
K^K(T_{\theta}^*(X)) \ar[r,"p_*"] & K^K(\cN_{\theta})
\end{tikzcd}
\end{center}
\end{lemma}

\begin{proof}
This is where we use that $G(\RR)$ is split. Since split, we have that codimensions match up. Then use proper base change or something.
\end{proof}

This lemma reduces to showing the following: let $U_{\CC} \subset X \times X$ and $U_{\RR} \subset X$, $U_{\RR} = U_{\CC} \cap X_{\Delta}$. WTS: for a local system $L$ on $U_{\CC}$, we have
%
$$\gr[j_!L|_{U_{\RR}}] = \iota^* \gr[j_!L]$$

Maybe this is general?



\begin{prop}
For each $(\lambda, \nu) \in X^*(H) \times \fh^*$ there is an identity in $K^K(\cN_{\theta})$\todo{replaced $R$ with $i^*$}
%
$$i^* \gr [I_{\CC}(\lambda,\nu)] = \gr [I_{\RR}(\overline{\lambda},\nu)].$$
\end{prop}

\begin{proof}
By Theorem \ref{thm:grprincipal}
%
$$\gr[I_{\CC}(\lambda,\nu)] = p_*([\pi^*\cO_{X \times X}(\delta, \delta)] \otimes [p^*\cO_{\fg^*_{-\Delta}}])$$
%
and
%
$$\gr[I_{\RR}(\overline{\lambda},\nu)] = p_*([\pi^*\cO_X(\delta)] \otimes [p^*\cO_{\fp^*}])$$
%
By Lemma ??
%
$$i^* \gr[I_{\CC}(\lambda,\nu)] = p_*\iota^*([\pi^*\cO_{X \times X}(\delta, \delta)] \otimes [p^*\cO_{\fg^*_{-\Delta}}])$$
%
Note that
%
\begin{align*}
\iota^*([\pi^*\cO_{X \times X}(\delta, \delta)] \otimes [p^*\cO_{\fg^*_{-\Delta}}]) &= \iota^*[\pi^*\cO_{X \times X}(\delta,\delta)] \otimes \iota^*[p^*\cO_{\fg^*_{-\Delta}}]\\
&= [\pi^*\cO_X(\delta)] \otimes p^*i^*[\cO_{\fg^*_{-\Delta}}]\\
&= [\pi^*\cO_X(\delta)] \otimes

\end{align*}
\end{proof}

\begin{lemma}
The map
%
$$\Theta_{\RR}: \Lambda \to KM_{fl}(G_{\RR}), \qquad \Theta_{\RR}(\gamma) = \mathcal{R}[I_{\CC}(\lambda+\gamma,\nu+\gamma)]$$
%
is a coherent family.
\end{lemma}

\begin{proof}
Define
%
$$\Theta_{\CC}: \Lambda \times \Lambda \to KM_{fl}(G), \qquad \Theta_{\CC}(\gamma,\gamma') = [I_{\CC}(\lambda+\gamma-\gamma',\nu+\gamma+\gamma')]$$
%
Clearly, $\Theta_{\CC}$ is a coherent family for $G$ (cf. \cite[Lemma 5.7]{SpehVogan}). For $\delta,\epsilon \in \Lambda$, write $F_{\CC}(\delta,\epsilon)$ for the (finite-dimensional) Langlands subquotient of $I_{\CC}(\delta,\epsilon)$. 






$F_{\CC}(\delta,\delta') = F(\delta-\delta') \otimes F(\delta+\delta')$ for the finite-dimensional irreducible in $M_{fl}(G)$, the Langlands quotient of $I_{\CC}(\delta,\delta')$. Then
%
$$I_{\CC}(\lambda+\gamma-\gamma',\nu + \gamma+\gamma') \otimes F_{\CC}(\delta,$$
%
In particular
%
\begin{equation}\label{eq:cohfamilies}[I_{\CC}(\lambda+\gamma,\nu+\gamma)] \otimes [F(\delta,\delta)] = \sum_{\mu \in F(\delta)} [I_{\CC}(\lambda+\gamma+\mu,\nu+\gamma+\mu)]\end{equation}
%
Note that $F(\delta,\delta)$ is a trivial $\fk_R$-module. So for any $X \in M(G)$
%
$$\mathcal{R}_i(X \otimes F_{\CC}(\delta,\delta)) \simeq \mathcal{R}_i(X) \otimes F(\delta)$$
%
Consequently
%
$$\mathcal{R}[X \otimes F_{\CC}(\delta,\delta)] = \mathcal{R}[X] \otimes [F(\delta)]$$
%
Applying $\mathcal{R}$ to both sides of (\ref{eq:cohfamilies}), we get
%
$$\mathcal{R}[I_{\CC}(\lambda+\gamma,\nu+\gamma)] \otimes [F(\delta)] = \sum_{\mu \in F(\delta)} \mathcal{R}[I_{\CC}(\lambda+\gamma+\mu,\nu+\gamma+\mu)]$$
%
This proves the assertion.
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:principalseries}]

\end{proof}


==> scratch2.tex <==


\section{Restriction of coherent sheaves}\label{sec:coherent}

\todo{maybe rewrite with $\cN \subset \fg_{-\Delta}$}In this section, I will briefly recall the main results from \cite{MBfunctions}. Choose a maximal compact subgroup $K_{\RR}$ of $G_{\RR}$ and let $\theta: G \to G$ be the corresponding Cartan involution. Let $K$ be the group of $\theta$-fixed points (i.e. the complexification of $K_{\RR}$). Write $\fg$,$\fk$ for the Lie algebras and let $\fp = \fg^{-d\theta}$. There is a Cartan decomposition
%
\begin{equation}\label{eq:Cartan}\fg = \mathfrak{k} \oplus \fp\end{equation}
%
Using (\ref{eq:Cartan}), we can identify $\fp^*$ with $(\fg/\fk)^*$, a subspace of $\fg^*$. Restriction along the closed embedding $\fp^* \subset \fg^*$ defines a right-exact functor
%
$$R: \mathrm{QCoh}^G(\fg^*) \to \mathrm{QCoh}^K(\fp^*)$$
%
Write
%
$$L_iR: \mathrm{QCoh}^G(\fg^*) \to \mathrm{QCoh}^K(\fp^*), \qquad i \geq 0$$
%
for the left derived functors. Taking global sections, the category $\mathrm{QCoh}^G(\fg^*)$ (resp. $\mathrm{QCoh}^K(\fp^*)$) can be identified with the category of $G$-equivariant $S(\fg)$-modules (resp. $K$-equivariant $S(\fp)$-modules), and $L_iR(M)$ can be identified with the $K$-equivariant $S(\fp)$-module $\mathrm{Tor}_i^{S(\fg)}(M,S(\fp))$. The latter can be computed using a standard Koszul complex
%
\begin{equation}\label{eq:Koszul1}0 \to \wedge^d(\fk) \otimes M \to \wedge^{d-1}(\fk) \otimes M \to ... \to \wedge^1(\fk) \otimes M \to M \to 0\end{equation}
%
Here $d = \dim(\fk)$ and the differentials are given by
%
\begin{align*}
\partial(X_1 \wedge ... \wedge X_n \otimes v) = &\sum_{i=1}^n (-1)^i (X_1 \wedge... \wedge \widehat{X}_i \wedge ... \wedge X_n \otimes X_iv)\\
+ &\sum_{j < k} (-1)^{j+k}([X_j, X_k] \wedge X_1 \wedge ... \wedge \widehat{X}_j \wedge ... \wedge \widehat{X}_k \wedge ... \wedge X_n \otimes v)\end{align*}
%
\begin{lemma}\label{lem:propsofRcommutative}
For each $i \geq 0$, the following are true:
\begin{itemize}
    \item[(i)] $L_iR$ restricts to a functor
    %
    $$L_iR: \Coh^G(\fg^*) \to \Coh^K(\fp^*).$$
    \item[(ii)] There is an isomorphism of $K$-equivariant $S(\fp)$-modules
    %
$$L_iR(M) \simeq H_i(\wedge(\fk) \otimes M)$$
\item[(iii)] If $i > d=\dim(\fk)$, then $L_iR=0$.
\item[(iv)] There is an inclusion of sets
%
$$\mathrm{Supp}(L_iR(M)) \subseteq \mathrm{Supp}(M) \cap \fp^*$$ 
\end{itemize}
\end{lemma}

Now let $\cN \subset \fg^*$ be the nilpotent cone and let $\cN_{\theta} = \cN \cap \fp^*$. Thanks to Lemma \ref{lem:propsofRcommutative}(i),(iv), there are functors
%
\begin{equation}\label{eq:LiRcommutative}L_iR: \Coh^G(\cN) \to \Coh^K(\cN_{\theta}), \qquad i \geq 0\end{equation}
%
Taking the alternating sum, we get a group homomorphism
%
\begin{equation}\label{eq:Rcommutative}R: K^G(\cN) \to K^K(\cN_{\theta}), \qquad R[M] = \sum_i (-1)^i [L_iR(M)].\end{equation}
%
(the sum on the right is finite thanks to Lemma \ref{lem:propsofRcommutative}(iii)). We explained in \cite{MBfunctions} how to compute this homomorphism. The group $\CC^{\times}$ acts by dilation on $\fg^*$ and this action preserves the subsets $\fp^*$, $\cN$, and $\cN_{\theta}$. There are graded versions of (\ref{eq:LiRcommutative}) and (\ref{eq:Rcommutative}) (denoted in the same way) and the following diagram commutes
\begin{center}
    \begin{tikzcd}
    K^G(\cN) \ar[r,"R"] & K^K(\cN_{\theta})\\
    K^{G \times \CC^{\times}}(\cN) \ar[r,"R"] \ar[u,twoheadrightarrow] & K^{K\times \CC^{\times}}(\cN_{\theta}) \ar[u,twoheadrightarrow]
    \end{tikzcd}
\end{center}

Let $\wedge(\fk)$ be the virtual finite-dimensional graded $K$-representation
%
$$\wedge(\fk) = \sum_i (-1)^i \wedge^i(\fk),$$
%
(with $\fk$ in degree $1$). Then the homomorphism $R:K^{G \times \CC^{\times}}(\cN) \to K^{K\times \CC^{\times}}(\cN_{\theta})$ is uniquely determined by the following identity of virtual graded $K$-representations
%
$$\Gamma(\cN_{\theta},R[M]) = \Gamma(\cN,[M]) \otimes \wedge(\fk)$$
%
This is \cite[Corollary 3.0.7]{MBfunctions}. We will also need the following.

\begin{prop}[Corollary 6.0.2, \cite{MBfunctions}]\label{prop:split}
Suppose $G_{\RR}$ is split modulo center. Then 
%
$$R[\cO_{\cN}] = [\cO_{\cN_{\theta}}].$$
\end{prop}




